Optimal Source-Based Filtering of Malicious Traffic

In this paper, we consider the problem of blocking malicious traffic on the Internet, via source-based filtering. In particular, we consider filtering via access control lists (ACLs): these are already available at the routers today but are a scarce resource because they are stored in the expensive ternary content addressable memory (TCAM). Aggregation (by filtering source prefixes instead of individual IP addresses) helps reduce the number of filters, but comes also at the cost of blocking legitimate traffic originating from the filtered prefixes. We show how to optimally choose which source prefixes to filter, for a variety of realistic attack scenarios and operators' policies. In each scenario, we design optimal, yet computationally efficient, algorithms. Using logs from Dshield.org, we evaluate the algorithms and demonstrate that they bring significant benefit in practice.

==> refs.tex <==


\begin{thebibliography}{99}


\bibitem{acl1} Cisco Systems, White Paper, ``Understanding
acl on catalyst 6500 series switches,''
{\em www.cisco.com/en/US/products/hw/switches/ps708/products \_white\_ paper09186a00800c9470.shtml. }

\bibitem{acl0} Cisco Systems, White Paper,
``Protecting your core: Infrastructure protection access control lists,''
{\em http://www.cisco.com/en/US/tech/tk648/tk361/technologies\_white \_paper09186a00801a1a55.shtml.}

\bibitem{dshield} Dshield {\em http://www.dshield.org/}



\bibitem{KPbook} H.Kellerer,U.Pferschy,D.Pisinger,``Knapsack Problems,'' Springer,2004.

\bibitem{varghese} G. Varghese, ``Network Algorithmics,'' Morgan Kaufmann, 2005.

\bibitem{infocom09} F.Soldo, A.Markopoulou, K.Argyraki, `Optimal Filtering of Source Address Prefixes: Models and Algorithm,''   {\em in Proc. of IEEE INFOCOM}, Rio de Janeiro, Brazil, April 2009.



\bibitem{GensLevner} G.V. Gens and E.V. Levner, ``Computational complexity of approximation algorithms for combinatorial problems,'' {\em in Mathematical
Foundations of Computer Science, LNCS}, vol. 74, pp.292-300, Springer 1979.


\bibitem{bertsekas} D.P. Bertsekas, ``Non linear programming,'' Athena Scientific, 2003.

\bibitem{boyd} S. Boyd,  L. Vandenberghe, ``Convex Optimization,'' Cambridge University Press, 2004.

\bibitem{clustering}Z.Chen, C.Ji, P.Barford, ``Spatial-Temporal Characteristics of Internet Malicious Sources,'' {\em in IEEE INFOCOM (Mini-Conf.)}, April 2008.

\bibitem{kohler} E. Kohler, J. Li, V. Paxson, and S. Shenker, ``Observed structure of addresses in IP
traffic,''{\em IEEE/ACM ToN 14(6)},pp.1207-1218,Dec.2006.

\bibitem{aitf} K. Argyraki, D.R.Cheriton, ``Active Internet
Traffic Filtering: Real-time Response to DoS
Attacks'', {\em in Proc. of USENIX Security 2005}.

\bibitem{xiaowei2} X. Liu, X. Yang, Y. Lu, ``To Filter or to Authorize: Network-Layer DoS Defense Against Multimillion-node Botnets,'' {\em in ACM SIGCOMM 2008}.%, Seattle, Aug.2008.

\bibitem{spoofer} R. Beverly, S. Bauer, ``The Spoofer Project: Inferring the Extent of Internet Source Address Filtering on the Internet,''{\em in SRUTI 2005}.


\bibitem{hipac} ``High Perf. Traffic Classification'',{\em www.hipac.org/performance\_tests/results.html}.


\bibitem{ingress} P.Ferguson,D.Senie,``Network Ingress Filtering: Defeating DoS Attacks which employ IP Source Address Spoofing'', {\em RFC 2827}, May 2000.

\bibitem{AIP}   D.Andersen,H.Balakrishnan,N.Feamster,T.Koponen,D.Moon,S.Shenker, ``Accountable Internet Protocol (AIP),'' {\em in ACM SIGCOMM 2008}, Seattle, Aug. 2008.

\bibitem{passport} X. Liu, A. Li, X. Yang, D. Wetherall, ``Passport: Secure and Adoptable Source Authentication, '' {\em  in Proc. USENIX/ACM NSDI 2008}.




\bibitem{estan} G. Pack, J. Yoon, E. Collins, C. Estan, ``On Filtering of DDoS Attacks Based on
Source Address Prefixes,'' {\em in Proc. of SecureComm}, Aug.2006.


\bibitem{firewalls} E. Al-Shaer et al., ``Firewall Policy Advisor Project,'' De Paul Univ. {\em http://www.mnlab.cs.depaul.edu/projects/SPA/}
\bibitem{firewalls1} E. Al-Shaer, H. Hamed, R. Boutaba and M. Hasan, ``Conflict Classification and Analysis of Distributed Firewall Policies,'' IEEE Journal on Selected Areas in Communications, 2005


\bibitem{ita08} F. Soldo, K. El Defrawy, A. Markopoulou, B. Krishnamurthy,
and K. v.d. Merwe, ``Filtering sources of unwanted traffic'' {\em in
Proc. of Inf. Theory and Applications Workshop}, UCSD, Jan. 2008.


\bibitem{review-dKP} A FrŽville,  ``The multidimensional 0Ð1 knapsack problem: An overview'',  {\em European Journal of Operational Research}, Elsevier, 2004


\bibitem{Caprara}  A. Caprara, H. Kellerer, U. Pferschy, and D. Pisinger, ``Approximation algorithms for knapsack problems with cardinality constraints'', European Journal of Operational Research, 123:333-345, 2000


\bibitem{old15KP} P.C. Gilmore, and R.E. Gomory, ``A linear programming approach to the cutting stock problem, part II'', {\em Operations Research}, 1964



\bibitem{1.5KP-GUB} A. Bagchi, N.Bhattacharyya, N.Chakravarti, ``LP relaxation of the two dimensional knapsack problem with box
and GUB constraints'', {\em European Journal of Operational Research}, Elsevier, 1994

\bibitem{dKP-GUB} V.C. Lia, G.L. Curry, ``Solving multidimensional knapsack problems with generalized
upper bound constraints using critical event tabu search,'' {\em Computers and Operations Research}, Elsevier, 2005


\bibitem{continuous-1.5KP} I.R. de Farias, G.L. Nemhauser, ``A polyhedral study of the cardinality constrained knapsack problem'', {\em in Math. Progr.}, Springer, 2002

%%% ordered %%%



%\bibitem{primed} P. Verkaik, O. Spatscheck, J. van der Merwe and
%A. Snoeren,  ``PRIMED: A Community-of-Interest-Based DDoS Mitigation
%System,'' {\em in  SIGCOMM Workshop on Large Scale Attack Defense
%(LSAD)}, Sept. 2006


\bibitem{barford}  P.Barford, R.Nowak, R. Willett Rebecca, V. Yegneswaran,
``Toward a Model for Sources of Internet Background Radiation,''
{\em in Proc. of the Passive and Active Measurement Conference (PAM '06)}, March, 2006.

\bibitem{uncleanness}  M. P. Collins, S. Faber, J.
Janies, R. Weaver, M. De Shon, ``Using Uncleanliness to Predict
Future Botnet Addresses,'' {\em in Proc. of ACm IMC 2007}, San
Diego, CA, Oct. 2007.

\bibitem{gatech} Z. Chen and C. Ji, ``Measuring Network-Aware Worm Spreading Ability,''
{\em in Proc. of IEEE INFOCOM 2007}.



\bibitem{megiddo-tamir} N.Megiddo and A.Tamiry, ``Linear Time Algorithms for Some Separable Quadratic Programming Problems'', {\em Operations Research Letters}, 1993.



%%%%%%%%%%%%%

%\bibitem{agrawal} Q. Dong, S. Banerjee, J. Wang, D. Agrawal, ``Wire Speed Packet Classification Without TCAMs: A Few More Registers (And A Bit of Logic) Are Enough,'' {\em in Proc. ACM Sigmetrics}, San Diego, CA, June 2007,


%\bibitem{hipac} ``High Perf. Traffic Classification'',{\em www.hipac.org/performance\_tests/results.html}.

\bibitem{complexity} MR Garey, DS Johnson, ``Computers and Intractability: A Guide to the Theory of NP-completeness,'' W.H.Freeman \& Co Ltd, 1979

\bibitem{dawn} S. Venkataraman, A. Blum, D. Song, S. Sen, O. Spatscheck, ``Tracking Dynamic Sources of Malicious Activity at Internet Scale,'' NIPS,  2009

\end{thebibliography} 
